A Multi-Step Richardson-Romberg Extrapolation Method For Stochastic Approximation

We obtain an expansion of the implicit weak discretization error for the target of stochastic approximation algorithms introduced and studied in [Frikha2013]. This allows us to extend and develop the Richardson-Romberg extrapolation method for Monte Carlo linear estimator (introduced in [Talay & Tubaro 1990] and deeply studied in [Pag{\`e}s 2007]) to the framework of stochastic optimization by means of stochastic approximation algorithm. We notably apply the method to the estimation of the quantile of diffusion processes. Numerical results confirm the theoretical analysis and show a significant reduction in the initial computational cost.

==> fcts-vincent.tex <==
\newcommand{\blackboard}[1]{\mathbf{#1}} 
\newcommand{\Q}{\blackboard{Q}}%		rationels
\newcommand{\R}{\blackboard{R}}%		reels
\newcommand{\N}{\blackboard{N}}%		entiers
\renewcommand{\P}{\blackboard{P}}%	 	probabilite
\newcommand{\E}{\blackboard{E}}% 		esperance
\renewcommand{\L}{\blackboard{L}}%	 	Lebesgue

\newcommand{\calig}[1]{\mathcal{#1}}
%\newcommand{\A}{\calig{A}}% 			generateur infinitesimal diff
\newcommand{\Ao}{\mathfrak{A}}% 		generateur infinitesimal 
\newcommand{\dom}{\calig{D}}%			domaine
%\newcommand{\B}{\calig{B}}%			boule
%\newcommand{\C}{\calig{C}}% 			continue
%\newcommand{\F}{\calig{F}}% 			filtration F
\newcommand{\G}{\calig{G}}% 			filtration G
\renewcommand{\H}{\calig{H}}% 			hypothese
%\newcommand{\M}{\calig{M}}% 			ensemble des matrices
%\newcommand{\I}{\calig{I}}% 			ensemble des mes. inv.
%\renewcommand{\U}{\mathcal{U}}%

\DeclareMathOperator{\Tr}{Tr}%	 		fonction trace
\DeclareMathOperator{\sgn}{sgn}%	 	fonction signe
\DeclareMathOperator{\var}{var}%	 	variance
\DeclareMathOperator{\corr}{cor}%	 	correlation
\DeclareMathOperator{\cov}{cov}%	 	covariance
\DeclareMathOperator{\Id}{Id}% 			identite
%\DeclareMathOperator{\supp}{supp}% 		support
\DeclareMathOperator{\ent}{Ent}%		entropie
\DeclareMathOperator{\oGamma}{\Gamma}% 		operateur carre du champ
\newcommand{\D}[2][]{%				operateur differentiel 
    \textup{D}^{%
    {\scriptscriptstyle #1 \!}} #2}
\renewcommand{\d}[1]{\textup{d} #1}% 	le dx de l'integrale
\newcommand{\od}[1]{\!\circ\!\d #1}%		le dx stratonovich
\newcommand{\dd}{\partial}%				la derivee partielle

\newcommand{\conv}{%				convergence
    \xrightarrow[\phantom{ a.s }]{}}
\newcommand{\convps}{%				convergence p.s.
    \xrightarrow[\phantom{ a.s }]{a.s}}
\newcommand{\convloi}{%				convergence en loi
    \xrightarrow[\phantom{ a.s }]{\calig{L}}}
\newcommand{\convproba}{%			convergence en proba
    \xrightarrow[\phantom{ a.s. }]{\P}}
\newcommand{\convLp}[1][p]{%			convergence dans L^p
    \xrightarrow[\phantom{ a.s }]{\L^{#1}}}
\newcommand{\convLpetps}[1][p]{%		convergence dans L^p et p.s.
    \xrightarrow[ a.s ]{\L^{#1}}}
\newcommand{\convet}{%				convergence etroite
    \Rightarrow}

\newcommand{\delimleft}[2]{\ifcase #1\or%	delimiteur gauche
    \bigl#2\or %
    \Bigl#2\or %
    \biggl#2\or %
    \Biggl#2\or %
    \left#2\fi}
\newcommand{\delimright}[2]{\ifcase #1\or%	delimiteur droite
    \bigr#2\or %
    \Bigr#2\or %
    \biggr#2\or %
    \Biggr#2\or %
    \right#2\fi}
\newcommand{\pa}[2][5]{% 			parentheses
    \delimleft{#1}{(} #2 \delimright{#1}{)}}
\newcommand{\br}[2][5]{%	 		crochets
    \delimleft{#1}{[} #2 \delimright{#1}{]}}
\newcommand{\ac}[2][5]{%			accolades
    \delimleft{#1}{\{} #2 \delimright{#1}{\}}}

\newcommand{\psca}[2][5]{%			produit scalaire
    {\delimleft{#1}{\langle} #2%
    \delimright{#1}{\rangle}}}
\newcommand{\abs}[2][5]{%			valeur absolue
    {\delimleft{#1}{\lvert} #2%
    \delimright{#1}{\rvert}}}
\newcommand{\norm}[2][5]{% 			norme
    {\delimleft{#1}{\lVert} #2%
    \delimright{#1}{\rVert}}}
\newcommand{\normLp}[3][5]{%			norme L^p
    \norm[#1]{#3}_{\scriptscriptstyle #2}}
\newcommand{\normsup}[2][5]{%			norme infinie
    \norm[#1]{#2}_{\scriptscriptstyle \infty}}

\newcommand{\normal}[2][5]{%			loi normale
    \calig{N}\! \pa[#1]{#2}}
\newcommand{\domin}[2][5]{%			dominee
    \calig{O}\! \pa[#1]{#2}}
\newcommand{\neglig}[2][5]{o\! \pa[#1]{#2}}% 	negligeable
\newcommand{\un}{%				indicatrice
    \boldsymbol{1}}
\newcommand{\ind}[2][5]{%			indicatrice
    \boldsymbol{1}_{\ac[#1]{#2}}}

\newcommand{\prob}[2][5]{%			probabilite
    \P \! \br[#1]{#2}}
\newcommand{\probs}[3][5]{%			proba sous
    \P_{#2} \! \br[#1]{#3}}
\newcommand{\probc}[3][5]{%			proba conditionnelle
    \P \! \br[#1]{#2%
    \delimleft{#1}{.}%
    \vphantom{#2}\vphantom{#3}%
    \delimright{#1}{\vert} #3}}
\newcommand{\esp}[2][5]{%			esperance
    \E \! \br[#1]{#2}}
\newcommand{\esps}[3][5]{%			esperance sous
    \E_{#2} \!\br[#1]{#3}}
\newcommand{\espc}[3][5]{%			esperance conditionnelle
    \E \! \br[#1]{#2%
    \delimleft{#1}{.} \vphantom{#2}\vphantom{#3}%
    \delimright{#1}{\vert} #3}}

\newcommand{\sfrac}[2]{%			jolie fraction 1/2 etc 
    {}^{\scriptstyle #1} \!/\!%
    {}_{_{\scriptstyle #2}}}
\newcommand{\ssfrac}[2]{%			jolie fraction en exposant
    {}^{\scriptscriptstyle #1} \!/\!%
    {}_{_{\scriptscriptstyle #2}}}

\newcommand{\seq}[2][0]{%			une suite 
    {\bigl( #2_n \bigr)}_{n \ge #1}}
\newcommand{\proc}[2][0]{%			un processus
    {\bigl( #2_t \bigr)}_{t \ge #1}}


%						des raccourcis en vrac
\newcommand{\Er}{\calig{E}}
\newcommand{\ut}{\underline{t}}
\newcommand{\us}{\underline{s}}
\newcommand{\uu}{\underline{u}}
%\newcommand{\ie}{\textit{i.e. }}%		i.e.
%\renewcommand{\le}{\leqslant}% 			<= plus beau
%\renewcommand{\ge}{\geqslant}%			>= plus beau
\newcommand{\ds}{\displaystyle}%		displaystyle
\newcommand{\ts}{\textstyle}%			textstyle

